Active Learning with Weak Supervision for Gaussian Processes

Annotating data for supervised learning can be costly. When the annotation budget is limited, active learning can be used to select and annotate those observations that are likely to give the most gain in model performance. We propose an active learning algorithm that, in addition to selecting which observation to annotate, selects the precision of the annotation that is acquired. Assuming that annotations with low precision are cheaper to obtain, this allows the model to explore a larger part of the input space, with the same annotation budget. We build our acquisition function on the previously proposed BALD objective for Gaussian Processes, and empirically demonstrate the gains of being able to adjust the annotation precision in the active learning loop.

==> Proposed/gp_bald.tex <==
\subsubsection{BALD for Gaussian Processes}
We can derive the BALD objective for Gaussian Processes using the differential entropy of a Gaussian random variable, given in \cref{eq:entr_gauss}. The first term in the acquisition function in \cref{eq:mi_bald}, follows from the predictive distribution (\cref{eq:gp_pred})
%
\begin{align*}
    \entropy{\Y \mid \X, \xtrain{n}, \ytrain{n}} \propto \log \big(\sigma_{*}^{2} + \sigma^2(X)\big) + \text{const.},
\end{align*}
%
and the second term is
%
\begin{align}
    \expectation_{\model \mid \xtrain{n}, \ytrain{n}}\big[\entropy{\Y \mid \X, \model}\big] \propto \log \big(\sigma^2(X)\big) + \text{const}.
\end{align}
%
% \expectation_{\model \mid \xtrain{n}, \ytrain{n}}[\log |\sigma^2|] = 
%
Hence, the full BALD objective for GPs is given by
\begin{align}
    \text{MI}(\Y;\model \mid \X, \xtrain{n}, \ytrain{n}) \propto \log \big(\sigma_{*}^{2} + \sigma^2(X)\big) - \log \big(\sigma^2(X)\big),
    %\label{eq:bald_gp}
\end{align}
%
as the constants cancel each other out.
